A Fast Bootstrap Algorithm for Causal Inference with Large Data

Estimating causal effects from large experimental and observational data has become increasingly prevalent in both industry and research. The bootstrap is an intuitive and powerful technique used to construct standard errors and confidence intervals of estimators. Its application however can be prohibitively demanding in settings involving large data. In addition, modern causal inference estimators based on machine learning and optimization techniques exacerbate the computational burden of the bootstrap. The bag of little bootstraps has been proposed in non-causal settings for large data but has not yet been applied to evaluate the properties of estimators of causal effects. In this paper, we introduce a new bootstrap algorithm called causal bag of little bootstraps for causal inference with large data. The new algorithm significantly improves the computational efficiency of the traditional bootstrap while providing consistent estimates and desirable confidence interval coverage. We describe its properties, provide practical considerations, and evaluate the performance of the proposed algorithm in terms of bias, coverage of the true 95% confidence intervals, and computational time in a simulation study. We apply it in the evaluation of the effect of hormone therapy on the average time to coronary heart disease using a large observational data set from the Women's Health Initiative.

==> old_text.tex <==
% partitions the full dataset of size $n$ into a certain number of subsets of size $b$. Then, bootstrap resamples of size $n$, the size of the full dataset, are done in each subsets.

% \subsection{Causal BLB}\label{sec:related}

% The causal bootstrap procedure from \cite{imbens2021causal} first imputes the potential outcomes for the treated and control group using an isotone copula. By Sklar's theorem, the joint potential outcome cdf $F_{01}$ of the treated and control groups can be written as $F_{01}(y_0, y_1) = C(F_0(y_0), F_1(y_1))$ for some copula $C: [0, 1] \times [0, 1] \rightarrow [0, 1]$ \cite[p. 1465]{imbens2021causal}. The authors show that assuming the potential outcomes are drawn from an \textit{isotone} coupling produces asymptotically conservative inference. The isotone coupling is given by $C^\textrm{iso}(u, v) = \min\{u, v \}$. Imputation using the isotone coupling produces the following imputed potential outcomes: \lw{(We need to make it clear that causal bootstrap first imputes the marginal distribution for the population and then impute the joint distribution with isotone. To save time or because of the big data setting, we don't impute the marginal to population. )}

% \begin{align}
% \tilde{Y}_i(0) &= \begin{cases} Y_i & \textrm{if } W_i = 0 \\ \hat{F}_0(\hat{F}_1^{-1}(Y_i)) & \textrm{otherwise} \end{cases} \\
% \tilde{Y}_i(1) &= \begin{cases} Y_i & \textrm{if } W_i = 1 \\ \hat{F}_1(\hat{F}_0^{-1}(Y_i)) & \textrm{otherwise} \end{cases}
% \end{align}

% For observational data, a balancing score is included in the imputation step through inclusion in the empirical cdfs as follows:

% \begin{align}
% \hat{F}_0(y_0|b) &= \dfrac{\frac{1}{nh^{-d_B}}\sum_{i=1}^n \mathbf{1}\{Y_i \leq y_0\}\frac{1-W_i}{1-e(X_i)}K\left(\frac{b(X_i) - b}{h}\right)}{\frac{1}{nh^{-d_B}}\sum_{i=1}^n\frac{1-W_i}{1-e(X_i)}K\left(\frac{b(X_i) - b}{h}\right)} \\
% \hat{F}_1(y_1|b) &= \dfrac{\frac{1}{nh^{-d_B}}\sum_{i=1}^n \mathbf{1}\{Y_i \leq y_1\}\frac{W_i}{e(X_i)}K\left(\frac{b(X_i) - b}{h}\right)}{\frac{1}{nh^{-d_B}}\sum_{i=1}^n\frac{W_i}{e(X_i)}K\left(\frac{b(X_i) - b}{h}\right)}
% \end{align}

% where $K$ is a kernel function and $h$ is the bandwidth\footnote{In the simulations, we use a standard Gaussian kernel with bandwidth $h = \frac{n}{2}^{-0.15}$}. By including the balancing score, we hope to satisfy the assumption of treatment ignorability which is usually obtained in randomized trials (see section \ref{sec:properties}). 

% In the case of the causal BLB, the algorithm psuedocode is shown in Algorithm \ref{alg:blb} and the algorithm is diagrammed in Figure \ref{fig:causalblbfig}. In words, the causal BLB first partitions the full dataset into $s$ distinct subsets and estimates a propensity score model and balancing score that is used in the imputation step. Imputation is done the same as in \citet{imbens2021causal}, where $(\tilde{Y}_i(0), \tilde{Y}_i(1))^n_{i=1}$ is estimated by the isotone coupling of the empirical cdfs. Using this imputation ensures conservative inference \citep{imbens2021causal}. Then, we simulate the randomization distribution within each subset by drawing a new randomization vector $\mathbf{W}^\ast$, summarize the resample estimates with a chosen statistic, and average that statistic across partitions to obtain an overall bootstrap estimate. Similar to the matching approach from \citet{otsu2017bootstrap}, we do not recalculate the IPW on the bootstrapped data, but sample them along with the observations. 

% \begin{algorithm}
% \begin{algorithmic}
% \For{$l \gets 1$ to $s$}
%     \State Calculate $n_1 = \sum_{i=1} W_i$ and $n_0 = n - n_1$
%     \State Sample a set of indices $I_l = \{i_1, \ldots, i_b\}$ from $\mathcal{I}$ without replacement
%     \State Set $\mathcal{I} = \mathcal{I}/\cap_{j = 1}^i I_j$
%     \State For the data $\mathbf{Y}_l = (Y_{i_1}, \ldots, Y_{i_b})$, construct a model of the propensity score $\hat{\pi}(X_i)$ and compute a balancing score $b(X_i)$.
%     \State Impute the potential outcomes by:
%     \begin{align}
% \tilde{Y}_i(0) &= \begin{cases} Y_i & \textrm{if } W_i = 0 \\ \hat{F}_0(\hat{F}_1^{-1}(Y_i)) & \textrm{otherwise} \end{cases} \\
% \tilde{Y}_i(1) &= \begin{cases} Y_i & \textrm{if } W_i = 1 \\ \hat{F}_1(\hat{F}_0^{-1}(Y_i)) & \textrm{otherwise} \end{cases} 
% \end{align}
% where $\hat{F}_0$ and $\hat{F}_1$ are nonparametric estimators of the control and treatment cdfs, respectively.
%     \For{$k \gets 1$ to $r$}
%         \State Sample $\left(M_1, \ldots, M_b\right) \sim \textrm{Multinomial}(n, \frac{1}{b}, \ldots, \frac{1}{b})$ 
%         \State Draw $W_1^\ast, \ldots, W_b^\ast$ i.i.d. from $\textrm{Bernoulli}(\hat{\pi}(X_i))$
%         \State Compute the treatment estimator
%         \[
%         \hat{\tau}^{(j)\ast}_k = \dfrac{b}{n}\displaystyle\sum_{i=1}^b \dfrac{W_i^\ast Y_i M_i}{\frac{\hat{\pi}(X_i)}{\sum W_i^\ast\hat{\pi}(X_i)}} - \dfrac{(1-W_i^\ast) Y_i M_i}{\frac{1- \hat{\pi}(X_i)}{\sum (1-W_i^\ast)\hat{\pi}(X_i)}} 
%         \]
%     \EndFor
%     \State $\hat{\tau}^{(l)} \gets \frac{1}{r}\sum_{i=1}^r \hat{\tau}_{i}^{(l)}$
% \EndFor
% \State $\hat{\tau}^\ast \gets \frac{1}{s}\sum_{i=1}^s \hat{\tau}^{(i)\ast}$
% \end{algorithmic}
% \caption{Causal BLB}
% \label{alg:blb}
% \end{algorithm}

% \begin{figure}
%     \centering
%     \includegraphics[scale = 0.62]{bootstrap.pdf}
%     \caption{Causal BLB}
%     \label{fig:causalblbfig}
% \end{figure}



% \begin{tikzpicture}[scale = 1, node distance = 1mm and 7mm,
% bootnode/.style={rectangle, draw=black!60, very thick, minimum size=5mm, align = center},
% fullnode/.style={rectangle, draw=black!60, very thick, minimum size=5mm},
% ellipse/.style={minimum size = 5mm}
% ]
% \node[fullnode] (main) {Original Data};
% \node[bootnode]        (subset1) [right=of main]   {Subset 1\\$(Y_i(1), Y_i(0)) \sim C^\textrm{iso}(\hat{F}_0, \hat{F}_1)$};
% \node (ellipse1) [below= of subset1] {$\vdots$};
% \node[bootnode]        (subset2) [below=of ellipse1]   {Subset $s$ \\$(Y_i(1), Y_i(0)) \sim C^\textrm{iso}(\hat{F}_0, \hat{F}_1)$};
% \draw[->] (main.east) -- (subset1.west);

% % \draw[draw=black] (-4, -1)rectangle(0, 2);
% % \draw(-2, 0.5) node {Original Data};
% % \draw[->] (0.1, 0.5) -- (0.6, 0.5);
% % \draw[draw=black] (1, 0.5) rectangle (5, 2);
% \end{tikzpicture}

%\ignore{
%\begin{assumption}[Consistency]
%If $W = w$, then $Y(w) = Y$
%\end{assumption}

%\begin{assumption}[Noninterference]
%Counterfactual outcomes for one unit do not depend on the %treatment values for other units
%\end{assumption}

%\begin{assumption}[Positivity]
%$P(W = w) > 0$
%\end{assumption}
%}







%The original BLB was developed in \citet{kleiner2014scalable}. The algorithm takes a subset size parameter $b$ and a desired number of subsets $s$ and constructs $s$ disjoint subsets of size $b$ each.\footnote{In this paper, we exhaustively partition the data into subsets, but it is not necessary to partition every observation into a subset, especially when the number of observations is large (see section \ref{sec:hyperparam}).} algorithm selects a certain number of subsets $s$ of size $b$. Then, for each subset, the algorithm takes $r$ bootstrap samples of size $n$, the full dataset, rather than size $b$, the size of the subset. The calculated bootstrap statistics are then averaged within each subset and then averaged across subsets.





%\subsection{Causal BLB}

% The causal BLB is a straightforward combination of the methods in \citet{imbens2021causal} and \citet{kleiner2014scalable}. As a result, favorable large-sample properties are obtained through small changes in the proofs (see section \ref{sec:proofs} for a review of the proofs).  We will show in the simulations and applied sections that the causal BLB algorithm works well in practice. However, the necessity for imputation causes the algorithm to be relatively slow for large datasets. As an alternative, we propose the weighted BLB algorithm shown in .


% \subsection{Properties}\label{sec:properties}

% \cite{imbens2021causal} showed that, for both observational and randomized trial data, the causal bootstrap procedure yields conservative inference. In particular, under the usual causal assumptions (see Assumptions 6.1-6.4 in \citet[pp. 1479-80]{imbens2021causal}), the confidence intervals are asymptotically valid: Let $F_{01}$ be the joint cdf of the treated and control potential outcomes and $\tau$ be a functional of $F_{01}$ (e.g., the ATE). 

% \begin{assumption}[Treatment Ignorability]
% \[
% (Y_i(0), Y_i(1)) \ind W_i | X_i
% \]
% \end{assumption}

% \begin{assumption}[Overlap]
% The propensity score $e(X_i) \equiv P(W_i = 1 | X_i)$ satisfies 
% \[0 < \min_{W_i = 1} e(X_i) \leq e(X_i) \leq \max_{W_i = 0} e(X_i) < 1 \]
% \end{assumption}

% \begin{assumption}[Superpopulation]
%  For each unit $i=1,\ldots,n$ in the population, attributes $X_i$ are i.i.d. draws from the distribution $F_X(x)$, and potential values of $Y_i(0), \, Y_i(1)$  are independent draws from the distribution $F_{01}(y_0, y_1 | x)$. $F_X$ and $F_{01}$ that are twice continuously differentiable in the continuously distributed components of $x$.

% \end{assumption}

% \begin{assumption}[Conditioning on $b(X_i)$]
% (a) We either have that $\mathcal{B}$ is a finite set $\{b_1, \ldots, b_k\}$ with $\mathbf{P}(b(X_i) = b_k) \geq p_B$ for each $k = 1, \ldots, K$ and some $p_B > 0$, or that $b(X_i)$ is continuously distributed on a set $\mathcal{B} \subset \mathbf{R}^{d_B}$ with density bounded away from zero. \\
% (b) If $b(X_i)$ is continuously distributed, the smoothing estimator uses a bandwidth $h=h_n$ satisfying $h_n \rightarrow 0$ and $nh_n^{d_B} \rightarrow \infty$. \\
% (c) The first four moments of the conditional distribution of $Y_i(0)$, $Y_i(1)$ given $b(X_i)$ are bounded almost surely. \\
% (d) The conditional distribution given the balancing score $F_{01}(y_0, y_1|b)$ has a bounded pdf $f_{01}(y_0, y_1|b)$ that is twice continuously differentiable in the continuously distributed components of $b(X_i)$.
% \end{assumption}

% \begin{theorem}[Observational Confidence Intervals]
% Under Assumptions 4-7, the bootstrap confidence intervals are asymptotically valid, i.e.:

% \[
% \lim_{n} \inf_{F_{01}} \mathbf{P}_{F_{01}}(\tau(F_{01}) \in \textrm{CI}(1-\alpha)) \geq 1 - \alpha
% \]
% \end{theorem}

% This result is established in \citet{imbens2021causal} through the derivation of two central limit theorem results, one governing the drawing of observations from the population to the sample, and the second dealing with the bootstrapping procedure. Because we share the imputation procedure from the causal bootstrap procedure, we can appeal to the same proofs \citet{imbens2021causal} once we show that our BLB process converges to same process as the causal bootstrap (see section \ref{sec:proofs}).



%1. consistency
%2. complexity
%3. appendix results (close connection with our algorithm and Imbens bootstrapping)
%4. data-structure agnostic (trial and observational data)

%For the causal BLB, we show in appendix  \ref{sec:consistent} that the weighted BLB estimator behaves similarly to the variance-stabilized IPW estimator; in particular, we show that it converges in probability to the IPW estimator. Therefore, in any analysis where the IPW estimator is appropriate, the causal BLB works as well.




% \begin{itemize}

%     \item[1] Construct IPW weights $w(X_i)$ in the full sample and construct weighted empirical cdfs for the potential outcomes, $\hat{F}_1(y_1) = \frac{\sum_{i=1}^n W_iw(X_i)\mathbf{1}(Y_i \leq y_1)}{\sum_{i=1} W_i w(X_i)}$ and $\hat{F}_0(y_0) = \frac{\sum_{i=1}^n (1-W_i)w(X_i)\mathbf{1}(Y_i \leq y_0)}{\sum_{i=1} (1-W_i) w(X_i)}$
%     \item[3] Impute on potential outcomes in this sample using the isotone coupling \cite{imbens2021causal}:
%     \begin{align}
% \tilde{Y}_i(0) &= \begin{cases} Y_i & \textrm{if } W_i = 0 \\ \hat{F}_0(\hat{F}_1^{-1}(Y_i)) & \textrm{otherwise} \end{cases} \\
% \tilde{Y}_i(1) &= \begin{cases} Y_i & \textrm{if } W_i = 1 \\ \hat{F}_1(\hat{F}_0^{-1}(Y_i)) & \textrm{otherwise} \end{cases} \\
% \end{align}
%     \item[3] Partition the data and for each subset, for each bootstrap construct a new treatment assignment vector $\mathbf{W}^\ast$ and calculate the mean difference using the $\tilde{Y}$s.
% \end{itemize}
